Scalable and Safe Remediation of Defective Actions in Self-Learning Conversational Systems

Off-Policy reinforcement learning has been a driving force for the state-of-the-art conversational AIs leading to more natural humanagent interactions and improving the user satisfaction for goal-oriented agents. However, in large-scale commercial settings, it is often challenging to balance between policy improvements and experience continuity on the broad spectrum of applications handled by such system. In the literature, off-policy evaluation and guard-railing on aggregate statistics has been commonly used to address this problem. In this paper, we propose a method for curating and leveraging high-precision samples sourced from historical regression incident reports to validate, safe-guard, and improve policies prior to the online deployment. We conducted extensive experiments using data from a real-world conversational system and actual regression incidents. The proposed method is currently deployed in our production system to protect customers against broken experiences and enable long-term policy improvements.

==> backup.tex <==

% \begin{enumerate}
%     \item \textbf{Regression Sample}: an utterance that was routed to a hypothesis which resulted in undesirable user experience or responses that are inconsistent with the expected agent behavior. In other words, any misroute can be considered as a regression case.
%     \item \textbf{Progression Sample}: We define a progression sample is an utterance that was routed to a satisfactory candidate resulting in the desirable customer experience or the intended agent behavior. This is usually a complementary and contrasting example provided alongside a regression sample to convey the desired agent behavior. 
% \end{enumerate}
% \begin{equation}
%       o_{i}(X)=\begin{cases}
%     1, & \text{if $X \sim r_i, \forall r_i \in R_i$}.\\
%     0, & \text{otherwise}.
%   \end{cases}
% \end{equation}
% The traffic filtered by $o_i$ is then redirected to a hand-crafted policy behavior derived from the progression samples, denoted as $\gamma_i$, $\gamma_i \in \Gamma$. There is a one-to-one mapping between members of $O$ and $\Gamma$ as depicted in algorithm \ref{alg:mitigation}. 


% \mk{there is a gap as we jump into mitigation. We need to have a section on to define the problem and terms clearly before jumping to exact solution}


% This is done via fine-grained modeling and evaluation of an RL agents policy on the set of curated high-value samples that allows for scalable mitigation, remediation and guard-railing. We outline a how this system handles the end-to-end life cycle of a user-reported defect i.e. from mitigation to eventual assimilation into the model. 
%\mk{One key point missing from intro is explaining R and P and their purpose. We can go with not listing contributions for now. The ones we have right now are not really clear}
% Our contributions are as follows - 
% \begin{enumerate}
%     \item a system for careful curation of a dataset consisting of regression and progression samples (R/P dataset).
%     \item a strategy to use this dataset and evaluate a refreshed models predicted performance on the regression progression dataset (R/P evaluation).
%     \item a design for using the dataset and evaluation strategy to perform a best-case and worst case guard-railing of the system against the defects recurrence (R/P gating).
%     \item an approach for using data augmentation and updating the training pipeline for effective re-onboarding of offloaded traffic (R/P learning).
% \end{enumerate}
% These contributions are supplemented with qualitative and quantitative results from our experimentation on our commercial dataset and deployment. 

% old stuff
% \mk{I don't think we need all details in the following two paragraphs or even need to talk about self-learning. The reason we had these for other papers was that we wanted to present model arch, input featurese etc. which is not really the case for this paper.
% We can just introduce skill routing in the remove unnecessary stuff. Just simply saying there is a component that selects the best interpretation of an utterance (i.e. intent) routes customer request to skills. And this is a reinforcement learning model that is refreshed frequently using off-policy obj ...}
% Commercial conversational AI agents like Amazon Alexa, Apple Siri, Google Assistant and Microsoft Cortana have seen a tremendous improvement in their interactions with users which are getting more natural and seamless by the day \textbf{[*]}. These systems rely on a series of data driven machine learning components such automatic speech recognition (ASR), natural language understanding (NLU), skill routing, skill execution and text to speech (TTS) whose individual periodic improvements compound directly towards the overall performance of the AI agent. \textbf{Refer figure 1}. Even though these systems are better than ever before \textbf{[*]}, customers often report defects i.e. cases to the developers when the response from these systems don't meet their expectations \textbf{[*]}. In this work we outline a novel approach, deployed at scale, to handle the end-to-end life cycle of a customer-reported skill-routing defect i.e. right after mitigation to eventual assimilation into the model leveraging a handful of regression and progression samples provided by the customer.
% \begin{figure}[t]
%     \centering
%         \includegraphics[width=0.7\linewidth]{figures/No Image Available.png}
%         \caption{An overview of the major processing steps to handle a user request in a conversational system. Show it making an error. \mk{I think we do not really need Fig.1 or Fig.2. We can draw a big two-col drawing that shows overall approach e.g. RL model refreshes, deployment, mistakes, hot-fixes, evaluation, learning}}
%         \label{fig:conversation_system}
% \end{figure}
% bring focus on skill routing and self-learning
% \mk{We should have already explained it by this point. BTW, let's no directly say we focus on skill routing as our approach is more like a fix/remediate for off-policy RL models deployed in commercial systems regardless of what these models do or what features the consume}
% We focus on skill routing\footnote{\textbf{skill routing} is the process of using ASR and NLU outputs alongside contextual signals to select an appropriate skill and NLU interpretation to serve a request. When routed correctly, the selected skill is specialized to handle the request and provides an appropriate response for the user.} in particular but the approach can be extended to all other components of the AI agent. We build on top of work by \textbf{[*]} which leverages a self-learning approach based on contextual bandit learning for driving these regular skill-routing model improvements and updating its interaction policy \textbf{[*]}. 
% \mk{Let explain that each deployment improves overall performance but certain subpopulations and edge cases may regress which is not acceptable in a commercial system}
% \mk{defining unfamiliar stuff in footnote is not a good idea. Let's find a better word, maybe hot-fixing by curated expert rules? then call hot-fixing rules in the rest of the paper? I see no point in using the internal term for the paper} offloading\footnote{\textbf{offloading} is the process of redirecting traffic similar to customer-reported defects away from the machine learning model and into an alternate system, mostly hand-crafted rule based, in order to temporarily but immediately reduce business impact of the reported defects.} 
